Experience Selection Using Dynamics Similarity for Efficient Multi-Source Transfer Learning Between Robots

In the robotics literature, different knowledge transfer approaches have been proposed to leverage the experience from a source task or robot -- real or virtual -- to accelerate the learning process on a new task or robot. A commonly made but infrequently examined assumption is that incorporating experience from a source task or robot will be beneficial. In practice, inappropriate knowledge transfer can result in negative transfer or unsafe behaviour. In this work, inspired by a system gap metric from robust control theory, the $\nu$-gap, we present a data-efficient algorithm for estimating the similarity between pairs of robot systems. In a multi-source inter-robot transfer learning setup, we show that this similarity metric allows us to predict relative transfer performance and thus informatively select experiences from a source robot before knowledge transfer. We demonstrate our approach with quadrotor experiments, where we transfer an inverse dynamics model from a real or virtual source quadrotor to enhance the tracking performance of a target quadrotor on arbitrary hand-drawn trajectories. We show that selecting experiences based on the proposed similarity metric effectively facilitates the learning of the target quadrotor, improving performance by 62% compared to a poorly selected experience.

==> sections/gap_background.tex <==
\section{Background on Gap Metric (0.5)}
\label{sec:gap_metric}
% co-prime factorization etc.
% geometric interpretation of nu-gap and implication

==> sections/proposed_algorithm.tex <==
\section{Background}
\label{sec:background}
\textcolor{red}{Will rewrite/remove this section altogether upon finishing the main section.}
In this section, we provide background information on the $\nu$-gap metric, Bayesian Optimization.
% formulation
% GP and BO stuff
% algorithm and some discussion (e.g., error bound)
%
\subsection{Background on the $\nu$-Gap Metric (0.25)}
\label{subsec:gap_background}
    From robust control, a notion of system similarity is the $\nu$-gap metric, which gives a notion of `distance' between two linear systems. First introduced into the robust control literature in \cite{vinnicombe1993frequency}, it is used for stability analysis of plant and controller pairs subject to perturbations (cf. ~\cite{vinnicombe1993frequency,zhou1998essentials}). For two LTI SISO systems with transfer functions $P_1(s)$ and $P_2(s)$\textcolor{red}{ z}, the $\nu$-gap metric can be computed from (\cite{zhou1998essentials})
	%
% 	\begin{equation}
%     	\begin{split}
%         	\delta_\nu(P_1, P_2) &\defeq \sup_\omega \psi(P_1,P_2) \\
%         	&= \sup_\omega \frac{|P_1(j\omega)-P_2(j\omega)|}{\sqrt{1+ |P_1(j\omega)|^2}\sqrt{1+ |P_2(j\omega)|^2}}. 
%     	\end{split}
%     	\label{eq:vgap}
% 	\end{equation}
	\begin{equation}
        % 	\delta_\nu(P_1, P_2) \defeq \sup_\omega \psi(P_1(j\omega), P_2(j\omega)),
        \delta_\nu(P_1, P_2) \defeq \sup_\omega \psi(z_1(\omega), z_2(\omega)),
    	\label{eq:vgap}
	\end{equation}
	where $z_k(\omega) \defeq A_k(\omega)e^{j\theta_k(\omega)}$ ($k=1,2$) characterizes the magnitude ($A_k(\omega)$) and phase ($\theta_k(\omega)$) of the input/output response of system $k$ subject to an input of frequency $\omega$, and
	\begin{equation}
	   % \psi(P_1(j\omega), P_2(j\omega)) = \frac{|P_1(j\omega)-P_2(j\omega)|}{\sqrt{1+ |P_1(j\omega)|^2}\sqrt{1+ |P_2(j\omega)|^2}}.
	   \psi(z_1, z_2) = \frac{|z_1-z_2|}{\sqrt{1+ |z_1|^2}\sqrt{1+ |z_2|^2}}.
	    \label{eq:psi}
	\end{equation}
    \textcolor{red}{(discussion about the winding number)}
    \textcolor{red}{outline range of gap}
    
    The $\nu$-gap can be given a geometric interpretation in terms of projection onto the Riemann sphere, a unit sphere centered at $(0,0,0.5)$ tangent to the complex plane \cite{zhou1998essentials}. The point denoted by the solid red circle in Fig. \ref{fig:riemann_sphere} is projected onto the Riemann sphere as follows. A line is drawn between the point and the point $(0,0,1)$ (the \textit{North Pole}) on the sphere---the intersection of this line and the sphere (the open red dot in Fig. \ref{fig:riemann_sphere}) is its projection. The chordal distance between two points $z_1,z_2\in\mathbb{C}$ is the Euclidean distance between their projected points, and is given by Eqn. \eqref{eq:psi}. The $\nu$-gap (Eqn. \eqref{eq:vgap}) between two systems is the maximum chordal distance over all frequencies.
    
    % \begin{figure}
    % 	\centering
    % 	\includegraphics[width=0.45\textwidth,height=0.45\textheight,keepaspectratio]{figures/gap-illustration.png}
    % 	\vspace{1em}
    % 	\caption{Geometric interpretation of the $\nu$-gap metric (from \cite{zhou1998essentials}). Two points ($s_1, s_2$) are projected onto the Riemann sphere by connecting the points to the point $(0,0,1)$ on the sphere -- the intersection of these lines and the sphere is the projection of $s_1,s_2$. The chordal distance between the points $s_1, s_2$ is the Euclidean distance between their projected points, and is given by $\psi(s_1, s_2)$. \textcolor{red}{TODO better picture}} 
    % 	\label{fig:vgap-interpretation}
    % \end{figure} 
%
\subsection{Bayesian Optimization (0.25)}
\label{subsec:bo_background}

Bayesian optimization (BO) provides a method to maximize `black-box' functions -- i.e., functions for which we do not have an analytical expression for, and are computationally expensive to evaluate. BO uses a probabilistic model of the objective function $f$, and iteratively samples from this model to approximate the maximum of $f$ \cite{shahriari2015taking}. A common model for the objective function is a GP, with mean $\mu(x)$ and variance $\sigma(x)$ \cite{williams2006gaussian}. Given a set of samples $\mathcal{D}_n \defeq \{(x_1,f(x_1)), \dots, (x_n,f(x_n))\}$, we want the next point we sample at to improve upon (i.e., have a larger value) the samples we already have -- to determine the best point to sample at, it uses an \textit{acquisition function} $a(x)$, which defines a value of each point $x$ in the search space based on the past samples $\mathcal{D}_n$. A common acquisition function is the expected improvement (EI), which is defined for a point $x$ by $EI(x) \defeq \mathbb{E}\left[\text{max}(f(x) - f^*, 0)\right]$, where $f^* \defeq \max_{x_i} f(x_i)$ is the largest sample observed so far. It can be shown (cf. \cite{shahriari2015taking}) EI can be computed as
%
\begin{equation}
     EI(x) = \begin{cases}
        (\mu(x) - f^*)\Phi(Z) + \sigma(x)\phi(Z) & \sigma(x) \neq 0 \\
        0 & \sigma(x) = 0,
    \end{cases}
    \label{eq:ei}
\end{equation}
where $Z \defeq \frac{\mu(x) - f^*}{\sigma(x)}$, and $\Phi$ and $\phi$ are the cumulative distribution function and probability density function of the standard normal distribution, respectively. The function maximum is found through an iterative process---the next sample point is given by $x_{next} = \argmax_x a(x)$, we augment our dataset $\mathcal{D}_{n+1} = \mathcal{D}_n \cup \{(x_{next},f(x_{next}))\}$, and the process is repeated. We consider the algorithm converged once it samples close to the same point in several consecutive iterations.

